Backdoor Federated Learning by Poisoning Backdoor-Critical Layers

Federated learning (FL) has been widely deployed to enable machine learning training on sensitive data across distributed devices. However, the decentralized learning paradigm and heterogeneity of FL further extend the attack surface for backdoor attacks. Existing FL attack and defense methodologies typically focus on the whole model. None of them recognizes the existence of backdoor-critical (BC) layers-a small subset of layers that dominate the model vulnerabilities. Attacking the BC layers achieves equivalent effects as attacking the whole model but at a far smaller chance of being detected by state-of-the-art (SOTA) defenses. This paper proposes a general in-situ approach that identifies and verifies BC layers from the perspective of attackers. Based on the identified BC layers, we carefully craft a new backdoor attack methodology that adaptively seeks a fundamental balance between attacking effects and stealthiness under various defense strategies. Extensive experiments show that our BC layer-aware backdoor attacks can successfully backdoor FL under seven SOTA defenses with only 10% malicious clients and outperform the latest backdoor attack methods.

==> sections/backdoor-critical_layer.tex <==
\section{Observing Backdoor-critical Layers}

According to our observation, some layers are critical to the backdoor task. In Fig.~\ref{fig:mnist_LSA}, we first train a CNN model to converge, then train this model in the clean dataset and the poisoned dataset respectively to get a benign model and a malicious model. When we substitute one single layer in the benign model for the corresponding layer in the malicious model, Fig.~\ref{fig:b2m} shows that the absence of layers in the malicious model does not prevent backdoor attack except for the absence of \texttt{fc1.weight} layer. When the layer \texttt{fc1.weight} in malicious model is substituted by the benign layer \texttt{fc1.weight}, backdoor attack fails. Then we substitute malicious layers for corresponding layers in the benign model. Fig.~\ref{fig:m2b} shows that only the appearance of layer \texttt{fc1.weight} in the malicious model can cause the success of the backdoor attack. We believe some layers are \textit{backdoor-critical}. The absence of even one of the backdoor-critical layers can cause a drop in the backdoor success rate.

\begin{figure}[t]
  \centering
  \includegraphics[scale=0.31]{figs/fashion_mnist_layersubstitutionanalysis.pdf}
  \includegraphics[scale=0.31]{./figs/cnn_substitution.pdf}
%   \subfigure[]{
%   \includegraphics[scale=0.31]{figs/fashion_mnist_layersubstitutionanalysis.pdf}\label{fig:b2m}}
%   \subfigure[]{
%   \includegraphics[scale=0.31]{./figs/cnn_substitution.pdf}\label{fig:m2b}}
%   \vspace{-0.1in}
  \caption{(a) The changes in backdoor success rate (BSR) of the malicious model with a layer substituted from the benign model. (b) The changes of BSR of the benign model with layer(s) substituted from the malicious model (``All except \texttt{fc1.weight}'' indicates replacing all layers except the \texttt{fc1.weight} with layers from the malicious model).}
  \label{fig:m2b}
  %\todo{explain where are the other layers?}}
%   Layer substitution analysis of five-layer CNN trained on Fashion-MNIST, backdoor success rate (BSR)}
    \label{fig:mnist_LSA}
\end{figure}


\begin{figure}[t]
\includegraphics[scale=0.5]{figs/scatter.pdf}
\label{fig:time-related}
\caption{layer set change according to time}
\end{figure}




==> sections/design.tex <==
\section{Design}

